RAT: Adversarial Attacks on Deep Reinforcement Agents for Targeted Behaviors

Evaluating deep reinforcement learning (DRL) agents against targeted behavior attacks is critical for assessing their robustness. These attacks aim to manipulate the victim into specific behaviors that align with the attacker's objectives, often bypassing traditional reward-based defenses. Prior methods have primarily focused on reducing cumulative rewards; however, rewards are typically too generic to capture complex safety requirements effectively. As a result, focusing solely on reward reduction can lead to suboptimal attack strategies, particularly in safety-critical scenarios where more precise behavior manipulation is needed. To address these challenges, we propose RAT, a method designed for universal, targeted behavior attacks. RAT trains an intention policy that is explicitly aligned with human preferences, serving as a precise behavioral target for the adversary. Concurrently, an adversary manipulates the victim's policy to follow this target behavior. To enhance the effectiveness of these attacks, RAT dynamically adjusts the state occupancy measure within the replay buffer, allowing for more controlled and effective behavior manipulation. Our empirical results on robotic simulation tasks demonstrate that RAT outperforms existing adversarial attack algorithms in inducing specific behaviors. Additionally, RAT shows promise in improving agent robustness, leading to more resilient policies. We further validate RAT by guiding Decision Transformer agents to adopt behaviors aligned with human preferences in various MuJoCo tasks, demonstrating its effectiveness across diverse tasks.

==> tables/case_one_results.tex <==
\begin{table*}[!ht]
\vspace{-0.3em}
\centering
\caption{The average attack success rate, along with the standard deviation, is calculated for various evasion attacks against victim agents in both scenarios. The results are averaged over 30 episodes. Full results are available at Appendix~\ref{appendix:full_experiment_results}.}
\vspace{-0.7em}
\label{tab:case_one_results}
\resizebox{0.96\textwidth}{!}{
\begin{tabular}{c|l|ccccc|c}
\toprule
& \multicolumn{1}{c|}{Dataset} & PA-AD (oracle) & PA-AD & SA-RL (oracle) & SA-RL & Random & \ourmethod (ours) \\
\midrule
\parbox[t]{3mm}{\multirow{4}{*}{\pix\rotatebox[origin=c]{90}{\footnotesize{Manipulation}}}} & ~~
   door-lock-v2 & 4.50 \stdv{4.00} & 3.50 \stdv{6.63} & 76.50 \stdv{14.97} & 39.50 \stdv{30.48} & 0.00 \stdv{0.00} & 87.00 \stdv{10.00} \\ & ~~ 
 % door-unlock-v2 & 0.00 \stdv{0.00} & 0.00 \stdv{0.00} & 11.11 \stdv{13.43} & 0.56 \stdv{0.00} & 0.00 \stdv{0.00} & 97.00 \stdv{6.63} \\ & ~~ 
 % window-open-v2 & 0.00 \stdv{0.00} & 0.00 \stdv{0.00} & 30.00 \stdv{21.19} & 8.00 \stdv{15.13} & 0.00 \stdv{0.00} & 72.50 \stdv{19.62} \\ & ~~ 
window-close-v2 & 0.00 \stdv{0.00} & 0.50 \stdv{0.00} & 99.00 \stdv{3.00} & 23.50 \stdv{37.22} & 0.00 \stdv{0.00} & 72.50 \stdv{40.01} \\ & ~~ 
 % drawer-open-v2 & 0.00 \stdv{0.00} & 0.00 \stdv{0.00} & 100.00 \stdv{0.00} & 26.00 \stdv{27.28} & 0.00 \stdv{0.00} & 97.50 \stdv{4.00} \\ & ~~ 
drawer-close-v2 & 0.00 \stdv{0.00} & 0.00 \stdv{0.00} & 57.50 \stdv{18.00} & 4.00 \stdv{8.00} & 0.00 \stdv{0.00} & 76.00 \stdv{24.98} \\ & ~~ 
 % faucet-open-v2 & 1.50 \stdv{4.00} & 2.50 \stdv{4.00} & 63.50 \stdv{20.52} & 0.00 \stdv{0.00} & 0.00 \stdv{0.00} & 84.00 \stdv{21.19} \\ & ~~ 
faucet-close-v2 & 0.00 \stdv{0.00} & 0.00 \stdv{0.00} & 66.50 \stdv{16.85} & 4.50 \stdv{9.22} & 0.00 \stdv{0.00} & 91.00 \stdv{6.71} \\
\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\pix\rotatebox[origin=c]{90}{Opposite}}} & ~~ 
   door-lock-v2 & 9.50 \stdv{7.48} & 10.00 \stdv{9.17} & 8.00 \stdv{13.42} & 2.00 \stdv{0.00} & 1.00 \stdv{3.00} & 99.00 \stdv{3.00} \\ & ~~ 
 % door-unlock-v2 & 3.00 \stdv{5.00} & 4.00 \stdv{4.58} & 8.00 \stdv{18.33} & 6.00 \stdv{12.00} & 0.00 \stdv{0.00} & 98.50 \stdv{4.00} \\ & ~~ 
 % window-open-v2 & 15.50 \stdv{12.21} & 17.00 \stdv{11.14} & 15.00 \stdv{16.61} & 7.00 \stdv{16.12} & 1.00 \stdv{3.00} & 77.50 \stdv{33.41} \\ & ~~ 
window-close-v2 & 38.50 \stdv{23.69} & 55.00 \stdv{14.70} & 63.00 \stdv{34.70} & 20.00 \stdv{39.80} & 5.50 \stdv{5.00} & 99.00 \stdv{0.00} \\ & ~~ 
 % drawer-open-v2 & 1.50 \stdv{4.00} & 0.50 \stdv{3.00} & 1.11 \stdv{0.00} & 3.00 \stdv{0.00} & 0.00 \stdv{0.00} & 85.50 \stdv{29.34} \\ & ~~ 
drawer-close-v2 & 88.50 \stdv{7.81} & 79.00 \stdv{18.44} & 81.00 \stdv{20.88} & 63.00 \stdv{32.50} & 0.00 \stdv{0.00} & 92.00 \stdv{17.32} \\ & ~~ 
 % faucet-open-v2 & 6.50 \stdv{9.00} & 10.00 \stdv{13.75} & 6.00 \stdv{18.00} & 0.00 \stdv{0.00} & 0.00 \stdv{0.00} & 81.50 \stdv{29.68} \\ & ~~ 
faucet-close-v2 & 19.00 \stdv{13.27} & 32.00 \stdv{11.00} & 7.00 \stdv{12.81} & 8.00 \stdv{16.00} & 0.50 \stdv{0.00} & 96.00 \stdv{12.81} \\
\bottomrule
\end{tabular}
} % resize the talbe
\end{table*}

==> tables/component_contribution.tex <==
\begin{table*}[t]
\centering
\caption{Effects of each component in \ourmethod is evaluated based on the average attack success rate on four simulated robotic manipulation tasks. These results represent the mean success rate across five runs.}
% \vspace{-0.7em}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{cccccc}
    \toprule
    \textbf{Scenario} & \textbf{Task} & \textbf{\ourmethod} & \textbf{\ourmethod w/o $h_\omega$} & \textbf{\ourmethod w/o $\pi_\theta$} & \textbf{\ourmethod w/o combination}  \\
    \midrule
    \multirow{2}{*}{Manipulation} 
    & Drawer Open & \textbf{99.1\%} & 91.3\% & 21.7\% & 68.0\% \\
    & Drawer Close & \textbf{80.9\%} & 70.2\% & 8.0\% & 26.0\% \\
    \midrule
    \multirow{2}{*}{Opposite} 
    & Faucet Open   & 84.4\% & \textbf{89.8}\% & 0.0\%  & 57.0\% \\
    & Faucet Close    & \textbf{95.1\%} & 94.1\% & 13.0\%  & 59.1\% \\
    \bottomrule
\end{tabular}
}
\label{tab:abla_component}
% \vspace{-1.0em}
\end{table*}

==> tables/robust_all_results.tex <==
\begin{table*}[!ht]
\centering
\caption{Average episode rewards $\pm $ standard deviation of robust agents under different attack methods, and results are averaged across 100 episodes.}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{cccccc}
    \toprule
    \textbf{Task} & \textbf{Model} & \textbf{\ourmethod} & \textbf{PA-AD} & \textbf{SA-RL} & \textbf{Average Reward}  \\
    \midrule
    \multirow{4}{*}{Door Lock} 
    & BA-ATLA  & 874\stdv{444}  & 628\stdv{486}  & 503\stdv{120}  & \textbf{668} \\
    & BA-WocaR & 774\stdv{241}  & 527\stdv{512}  & 520\stdv{236}  & 607 \\
    & PA-ATLA  & 491\stdv{133}  & 483\stdv{15 }  & 517\stdv{129}  & 497 \\
    & ATLA-PPO & 469\stdv{11 }  & 629\stdv{455}  & 583\stdv{173}  & 545 \\
    \midrule
    \multirow{4}{*}{Door Unlock} 
    & BA-ATLA  & 477\stdv{203} & 745\stdv{75}  & 623\stdv{60}  & \textbf{615} \\
    & BA-WocaR & 525\stdv{78}  & 647\stdv{502} & 506\stdv{39}  & 559 \\
    & PA-ATLA  & 398\stdv{12}  & 381\stdv{11}  & 398\stdv{79}  & 389 \\
    & ATLA-PPO & 393\stdv{36}  & 377\stdv{8}   & 385\stdv{26}  & 385 \\
    \midrule
    \multirow{4}{*}{Faucet Open} 
    & BA-ATLA  & 442\stdv{167} & 451\stdv{96}    & 504\stdv{55}   & 465 \\
    & BA-WocaR & 1223\stdv{102}& 1824\stdv{413}  & 1575\stdv{389} & \textbf{1541}\\
    & PA-ATLA  & 438\stdv{53}  & 588\stdv{222}   & 373\stdv{32}   & 466 \\
    & ATLA-PPO & 610\stdv{293} & 523\stdv{137}   & 495\stdv{305}  & 522 \\
    \midrule
    \multirow{4}{*}{Faucet Close} 
    & BA-ATLA  & 1048\stdv{343} & 1223\stdv{348} & 570\stdv{453}  & 947 \\
    & BA-WocaR & 1369\stdv{158} & 1416\stdv{208} & 3372\stdv{1311}& \textbf{2052}\\
    & PA-ATLA  & 661\stdv{279}  & 371\stdv{65}   & 704\stdv{239}  & 538 \\
    & ATLA-PPO & 1362\stdv{149} & 688\stdv{196}  & 426\stdv{120}  & 825 \\
    \bottomrule
\end{tabular}
}
\label{tab:robust2}
\vspace{-1.0em}
\end{table*}

==> tables/robust_all_results_single_col.tex <==
\begin{table}[!ht]
\centering
\caption{Average episode rewards $\pm $ standard deviation of robust agents under different attack methods, and results are averaged across 100 episodes.}
\vspace{-0.8em}
\resizebox{1.01\linewidth}{!}{
\begin{tabular}{ccccccc}
    \toprule
    \textbf{Task} & \textbf{Model} & \textbf{\ourmethod} & \textbf{PA-AD} & \textbf{SA-RL} & \textbf{Avg R}  \\
    \midrule
    % \multirow{4}{*}{Door Lock} 
    \parbox[t]{2mm}{\multirow{4}{*}{\pix\rotatebox[origin=c]{90}{Door Lock}}}
    & RAT-ATLA  & 874\stdv{444}  & 628\stdv{486}  & 503\stdv{120}  & \textbf{668} \\
    & RAT-WocaR & 774\stdv{241}  & 527\stdv{512}  & 520\stdv{236}  & 607 \\
    & PA-ATLA  & 491\stdv{133}  & 483\stdv{15 }  & 517\stdv{129}  & 497 \\
    & ATLA-PPO & 469\stdv{11 }  & 629\stdv{455}  & 583\stdv{173}  & 545 \\
    \midrule
    % \multirow{4}{*}{Door Unlock} 
    \parbox[t]{2mm}{\multirow{4}{*}{\pix\rotatebox[origin=c]{90}{\footnotesize{Door Unlock}}}}
    & RAT-ATLA  & 477\stdv{203} & 745\stdv{75}  & 623\stdv{60}  & \textbf{615} \\
    & RAT-WocaR & 525\stdv{78}  & 647\stdv{502} & 506\stdv{39}  & 559 \\
    & PA-ATLA  & 398\stdv{12}  & 381\stdv{11}  & 398\stdv{79}  & 389 \\
    & ATLA-PPO & 393\stdv{36}  & 377\stdv{8}   & 385\stdv{26}  & 385 \\
    \midrule
    % \multirow{4}{*}{Faucet Open} 
    \parbox[t]{2mm}{\multirow{4}{*}{\pix\rotatebox[origin=c]{90}{\footnotesize{Faucet Open}}}}
    & RAT-ATLA  & 442\stdv{167} & 451\stdv{96}    & 504\stdv{55}   & 465 \\
    & RAT-WocaR & 1223\stdv{102}& 1824\stdv{413}  & 1575\stdv{389} & \textbf{1541}\\
    & PA-ATLA  & 438\stdv{53}  & 588\stdv{222}   & 373\stdv{32}   & 466 \\
    & ATLA-PPO & 610\stdv{293} & 523\stdv{137}   & 495\stdv{305}  & 522 \\
    \midrule
    % \multirow{4}{*}{Faucet Close} 
    \parbox[t]{2mm}{\multirow{4}{*}{\pix\rotatebox[origin=c]{90}{\footnotesize{Faucet Close}}}}
    & RAT-ATLA  & 1048\stdv{343} & 1223\stdv{348} & 570\stdv{453}  & 947 \\
    & RAT-WocaR & 1369\stdv{158} & 1416\stdv{208} & 3372\stdv{1311}& \textbf{2052}\\
    & PA-ATLA  & 661\stdv{279}  & 371\stdv{65}   & 704\stdv{239}  & 538 \\
    & ATLA-PPO & 1362\stdv{149} & 688\stdv{196}  & 426\stdv{120}  & 825 \\
    \bottomrule
\end{tabular}
}
\label{tab:robust2_single}
\vspace{-1.0em}
\end{table}

==> tables/robust_part_results.tex <==
\begin{table}[t]
\centering
\caption{Average episode rewards $\pm$ standard deviation of robust agents under different attack methods, and results are averaged across 100 episodes. \fengshuo{Attention ref!} And all results (4 tasks) can be found in Appendix~\ref{appendix:}}
\resizebox{1.03\linewidth}{!}{
\begin{tabular}{ccccccc}
    \toprule
    \textbf{Task} & \textbf{Model} & \textbf{\ourmethod} & \textbf{PA-AD} & \textbf{SA-RL} & \textbf{Avg R}  \\
    \midrule
    % {\multirow{4}{*}{Door Lock} }
    \parbox[t]{2mm}{\multirow{4}{*}{\pix\rotatebox[origin=c]{90}{Door Lock}}}
    & BA-ATLA  & 874\stdv{444}  & 628\stdv{486}  & 503\stdv{120}  & \textbf{668} \\
    & BA-WocaR & 774\stdv{241}  & 527\stdv{512}  & 520\stdv{236}  & 607 \\
    & PA-ATLA  & 491\stdv{133}  & 483\stdv{15 }  & 517\stdv{129}  & 497 \\
    & ATLA-PPO & 469\stdv{11 }  & 629\stdv{455}  & 583\stdv{173}  & 545 \\
    \midrule
    % \multirow{4}{*}{Door Unlock} 
    \parbox[t]{2mm}{\multirow{4}{*}{\pix\rotatebox[origin=c]{90}{\footnotesize{Door Unlock}}}}
    & BA-ATLA  & 477\stdv{203} & 745\stdv{75}  & 623\stdv{60}  & \textbf{615} \\
    & BA-WocaR & 525\stdv{78}  & 647\stdv{502} & 506\stdv{39}  & 559 \\
    & PA-ATLA  & 398\stdv{12}  & 381\stdv{11}  & 398\stdv{79}  & 389 \\
    & ATLA-PPO & 393\stdv{36}  & 377\stdv{8}   & 385\stdv{26}  & 385 \\
    \bottomrule
\end{tabular}
}
\label{tab:robust}
\vspace{-1.0em}
\end{table}
